Federated Recommendation via Hybrid Retrieval Augmented Generation

Federated Recommendation (FR) emerges as a novel paradigm that enables privacy-preserving recommendations. However, traditional FR systems usually represent users/items with discrete identities (IDs), suffering from performance degradation due to the data sparsity and heterogeneity in FR. On the other hand, Large Language Models (LLMs) as recommenders have proven effective across various recommendation scenarios. Yet, LLM-based recommenders encounter challenges such as low inference efficiency and potential hallucination, compromising their performance in real-world scenarios. To this end, we propose GPT-FedRec, a federated recommendation framework leveraging ChatGPT and a novel hybrid Retrieval Augmented Generation (RAG) mechanism. GPT-FedRec is a two-stage solution. The first stage is a hybrid retrieval process, mining ID-based user patterns and text-based item features. Next, the retrieved results are converted into text prompts and fed into GPT for re-ranking. Our proposed hybrid retrieval mechanism and LLM-based re-rank aims to extract generalized features from data and exploit pretrained knowledge within LLM, overcoming data sparsity and heterogeneity in FR. In addition, the RAG approach also prevents LLM hallucination, improving the recommendation performance for real-world users. Experimental results on diverse benchmark datasets demonstrate the superior performance of GPT-FedRec against state-of-the-art baseline methods.

==> 6_ethics_statement.tex <==
\section*{Ethics Statement}
Our work provides a data-efficient and privacy-aware solution to address the open-vocabulary problem in federated learning. Our method automatically generalizes to a new user and is capable of answering her/his queries that involve data from novel categories. \huimin{In terms of real-world applications, with \ours, the update frequency of the deployed FL model could be drastically reduced, and there is no need to collect huge amount of training data for novel classes. The above two advantages of \ours reduce the risk of collecting private user data.}


% This is beneficial in real-world applications, since keeping updating the system is infeasible due to the huge amount of potential users, and our method could rescue.


==> tables/3_prompts.tex <==
\begin{table}[t]
\small
\begin{tabular}{@{}lll@{}}
\toprule
\textbf{Type}  & \textbf{Prompts}  \\ 
\midrule
\multirow{4}{*}{{\makecell{biased \\ prompts}}} 
& \texttt{A photo of a male, and he is [smiling].} \\
& \texttt{A photo of a female, and she is [smiling].} \\
& \texttt{A photo of a male, and he is [not smiling].} \\
& \texttt{A photo of a female, and she is [not smiling].} \\
\midrule
\multirow{2}{*}{{\makecell{unbiased \\ prompts}}} 
& \texttt{A photo of a [smiling] person.} \\
& \texttt{A photo of a [not smiling] person.} \\
\midrule
\multirow{2}{*}{{\makecell{demo.-only \\ prompts}}} 
& \texttt{A photo of a male.} \\
& \texttt{A photo of a female.} \\
\bottomrule
\end{tabular}
\caption{Crafted prompts for the CelebA smiling detection application. With biased prompts, CLIP achieves zero-shot accuracy of 84.8\% whereas with unbiased prompts, the zero-shot accuracy is only 74.8\%. Therefore, we choose to use the biased prompts in our experiments.}
\label{tab:prompts}
\vspace{-0.8cm}
\end{table}

